Towards a Model Theory of Ordered Logics: Expressivity and Interpolation (Extended version)

We consider the family of guarded and unguarded ordered logics, that constitute a recently rediscovered family of decidable fragments of first-order logic (FO), in which the order of quantification of variables coincides with the order in which those variables appear as arguments of predicates. While the complexities of their satisfiability problems are now well-established, their model theory, however, is poorly understood. Our paper aims to provide some insight into it. We start by providing suitable notions of bisimulation for ordered logics. We next employ bisimulations to compare the relative expressive power of ordered logics, and to characterise our logics as bisimulation-invariant fragments of FO a la van Benthem. Afterwards, we study the Craig Interpolation Property~(CIP). We refute yet another claim from the infamous work by Purdy, by showing that the fluted and forward fragments do not enjoy CIP. We complement this result by showing that the ordered fragment and the guarded ordered logics enjoy CIP. These positive results rely on novel and quite intricate model constructions, which take full advantage of the "forwardness" of our logics.

==> sections/lostarski.tex <==
%!TEX root = ../icalp2022.tex

\section{Preservation Theorems}\label{sec:lostarski}



==> sections/subsec-IEP.tex <==
%!TEX root = ../icalp2022.tex
%
\newcommand{\mosaicm}{\mathfrak{m}}
\newcommand{\mosaicn}{\mathfrak{n}}
\newcommand{\mosaicp}{\mathfrak{p}}
\newcommand{\mosaicsM}{\mathcal{M}}
\newcommand{\mosaicsP}{\mathcal{P}}
\newcommand{\mosaicsN}{\mathcal{N}}
\newcommand{\unarytype}{\mathfrak{u}}
\newcommand{\typet}{\mathfrak{t}}
\newcommand{\setofunarytypes}{\mathcal{U}}
\newcommand{\unfold}[1]{\llbracket #1 \rrbracket}
\newcommand{\mas}{\textrm{mx}_{\sigma}}

The rest of this subsection is dedicated to the proof of:
\begin{theorem}\label{thm:IEP-in-TOWER}
Joint-consistency of $\varphi$ and $\psi$ in $\Lsuffix/\Linfix$ is decidable in $\Tower$.
\end{theorem}
% %
W.l.o.g. we assume that $\varphi$ and $\psi$ are in $\Lsuffix$, in the normal form \ref{NForm-FL}.
Let $\tau := \sig(\varphi) \cap \sig(\psi)$, $\sigma := \sig(\varphi) \cup \sig(\psi)$ and let $\mas$ be the maximal arity of symbols in $\sigma$.
We will also use $\sigma_\ell$ to denote the restriction of $\sigma$ to symbols of arity $\leq \ell$.
For brevity, we write $\str{A}, \domelema \sim \str{B}, \domelemb$ if there exists an $\Lsuffix[\tau]$-bisimulation $\bisimZ \subseteq (A \times B)$ satisfying $(\domelema, \domelemb) \in \bisimZ$.
We write $\domelema \sim \domelemb$ if the structures $\str{A}, \str{B}$ can be deduced from the context.
Let $\Xi$ be composed of $\varphi, \psi$ and $\relsymbolR(\varx_1)$ for all unary $\relsymbolR \in \sigma$. 
We close $\Xi$ under a single negation and under subformulae, and define a \emph{unary type} as the maximally consistent subset of formulae from (the closed) $\Xi$. 
The denote the set of all unary types we use $\setofunarytypes$.
The unique unary type realised (defined in the expected way) by $\domelema$ in $\str{A}$ is denoted by $\unarytype_{\str{A}}(\domelema)$.

Henceforth assume that $\varphi, \psi$ are jointly-$\logicL[\tau]$-consistent and that they have $\logicL[\tau]$-bisimilar models $\str{A}_1, \str{A}_2$, with disjoint domains, witnessing it. 
W.l.o.g. every unary type realised in $\str{A}_1$ and $\str{A}_2$ is realised more than once (as $\logicL$ is an equality-free fragment of $\FO$). 
We aim at extracting  $\mathcal{O}(|\varphi|{+}|\psi|)$-fold exponential models $\str{B}_1 \models \varphi$ and $\str{B}_2 \models \psi$ satisfying $\str{B}_1 \sim \str{B}_2$.\\

\noindent \textbf{Mosaics.}
We follow the methodology from~\cite[Sec. VI]{JungW21}, adapting their construction for~$\FO^2$.
A \emph{mosaic} $\mosaicm = (\Phi_1, \Phi_2) \in 2^{\setofunarytypes} \times 2^{\setofunarytypes}$ is a pair of sets of unary types. 
Note that the number of different mosaics is exponential in the number of unary types, hence also exponential in $|\varphi|{+}|\psi|$.
The mosaic $\mosaicm(\domelema) = (\Phi_1, \Phi_2)$ \emph{generated by} $\domelema \in A_1 \cup A_2$ is defined with $\Phi_i = \{ \unarytype_{\str{A}_i}(\domelemd) \mid \domelemd \in A_i \ \text{and}\ \domelema \sim \domelemd \}$ for $1 \leq i \leq 2$.
The set $\mosaicsM$ of all mosaics is defined as $\{ \mosaicm(\domelema) \mid \domelema \in A_1 \cup A_2 \}$.
Intuitively, mosaics from $\mosaicsM$ tell us which "bisimilarity-preserving" types should be realised in the forthcoming structures.
For technical reasons we distinguish the sets of \emph{noble} and \emph{plebeian} mosaics, corresponding to pawn and king mosaics from~\cite{JungW21}.
A mosaic $\mosaicm$ is \emph{noble} if all the elements generating $\mosaicm$ are bisimilar, \ie for all $\domelemd, \domeleme$ such that $\mosaicm = \mosaicm(\domelemd) = \mosaicm(\domeleme)$ we have~$\domelemd \sim \domeleme$. 
Otherwise we call $\mosaicm$ \emph{plebeian}.
Note that noble mosaics may occur in $\str{A}_1$ and $\str{A}_2$, even if we require that $\str{A}_i$ realise every unary type more than once.
The sets of noble and plebeian mosaics are denoted with $\mosaicsN$ and $\mosaicsP$, and we use, respectively, $\mosaicn$ and $\mosaicp$ to denote their~elements.\\

\noindent \textbf{Construction of small models.} 
Let $K$ be \myundef{sufficiently large}, \eg it suffices to take \myundef{$K = ???$.}  
The domains $B_i$ of $\str{B}_1$ and $\str{B}_2$ will be defined simultaneously and are composed of:
\begin{itemize}\itemsep0em
  \item \emph{knights}, \ie elements of the form $((\unarytype, c_2, c_3, \ldots, c_{\mas}), \mosaicn)$, where $\mosaicn = (\Phi_1, \Phi_2)$ is a noble mosaic with $\unarytype \in \Phi_i$,
  \item \emph{peasants}, \ie elements of the form $((\unarytype, c_2, c_3, \ldots, c_{\mas}), (\mosaicp, c))$, where $\mosaicp = (\Phi_1, \Phi_2)$ is a plebeian mosaic with $\unarytype \in \Phi_i$,
\end{itemize}
where all $c$ range from $1$ to $K$. Such indices, called \emph{clocks}, will be employed later to assign $\ell$-ary relations ($c_\ell$ stored in the first coordinate) and to provide sufficiently many copies of plebeian mosaics ($c$ in the second coordinate).
We write $\unfold{\domelemb} = (\unarytype, \mosaicm)$ instead of $\domelemb = ((\unarytype, c_2, c_3, \ldots, c_{\mas}), \mosaicm)$ or $\domelemb = ((\unarytype, c_2, c_3, \ldots, c_{\mas}), (\mosaicm, c))$ whenever appropriate parameters $c$ exist.
We aim to ensure that the structures $\str{B}_1, \str{B}_2$ under construction satisfy:
\begin{description} \itemsep0cm 
  \item[\desclabel{(types)}{FL:types}] Every $\domelemb$ with $\unfold{\domelemb} = (\unarytype, \mosaicm)$ realises precisely $\unarytype$, \ie for all $\gamma(\varx_1) \in \setofunarytypes$ we have that $\str{B}_i \models \gamma(\domelemb)$ iff $\gamma(\varx_1) \in \unarytype$.
  %
  \item[\desclabel{(bisim)}{FL:bisim}] All \emph{copies} of $\mosaicm$ are bisimilar, \ie for all $\domelemb, \domelemb' \in B_{1} \cup B_{2}$ having their \emph{second coordinate} equal, we have $\domelemb \sim \domelemb'$.
\end{description} 

Having $B_i$ defined, we proceed with interpreting relational symbols from $\sigma$. 
We focus only on $\str{B}_1$ (to avoid too many subindices); the definition of $\str{B}_2$ is analogous.
Interpreting unary symbols is easy and we handle it in an expected way, \ie for $\domelemd$ with $\unfold{\domelemd} = (\unarytype, \mosaicm)$ we put $\domelemd \in \relsymbolR^{\str{B}_1}$ iff $\relsymbolR(\varx_1) \in \unarytype$.
Interpreting non-unary symbols is, however, involving: this explains why we have so many copies of domain elements. 
To do it, we will associate \emph{generators} and \emph{witnesses} and define non-unary relations according to them. 
Formally, we prepare:
\begin{itemize}\itemsep0em 
  \item a \emph{noble generator} $\domelemg_\mosaicn \in (A_1 \cup A_2)$ for each $\mosaicn \in \mosaicsN$, and \emph{plebeian generators} $\domelemg_{(\mosaicp, c)} \in (A_1 \cup A_2)$ \emph{per each copy} $(\mosaicp, c)$ of~$\mosaicp \in \mosaicsP$,
  \item for every $\domelemb$ with $\unfold{\domelemb} = (\unarytype, \mosaicm) \in B_1$ a \emph{witness} $\domelemw_\domelemb \in A_1$ satisfying $\unarytype = \unarytype_{\str{A}_1}(\domelemw_\domelemb)$ and $\domelemw_\domelemb \sim \domelemg$, where $\domelemg$ is the generator for the corresponding copy of $\mosaicm$ (\ie the second coordinate of $\domelemb$). 
 \end{itemize}

\noindent \textbf{Relations between knights.}
The choice of generators and witnesses for knights is not really important.
Thus for all noble mosaics $\mosaicn = (\Phi_1, \Phi_2) \in \mosaicsN$ we 
(1) select as their generator any $\domelemg_\mosaicn$ witnessing $\mosaicn = \mosaicm(\domelemg_\mosaicn)$, and
(2) for each $\unarytype \in \Phi_1$ we pick any $\domelemw_{(\unarytype, \mosaicn)} \in B_1$ (such an element exists by the definition of $\mosaicsM$) satisfying $\unarytype_{\str{A}_i}(\domelemw_{(\unarytype, \mosaicn)}) = \unarytype$ and $\mosaicm(\domelemw_{(\unarytype, \mosaicn)}) = \mosaicn$ as the \emph{witness for all} $\domelemb \in B_1$ satisfying $\unfold{\domelemb} = (\unarytype, \mosaicn)$.

In what follows, we define $\ell$-ary relations between knights inductively on $\ell \geq 1$. 
The case of $\ell = 1$ is already solved, so assume $\ell > 1$.
Take any noble mosaic $\mosaicn_1 = (\Phi_1, \Phi_2)$, a unary type $\unarytype_1 \in \Phi_1$ and $\ell{-}1$ knights $\domelemb_j = ( (\unarytype_j, \ldots), \mosaicn_j) \in B_j$ for $2 \leq j \leq \ell$.
We collect all $(\sigma_\ell,\ell)$-infix-types that are ``compatible'' with $\domelemtupleb$ by putting $L := $
\[ 
 \big\{ \tp{\Lsuffix[\sigma_\ell]}{\str{A}_1}{\domelemtupleafromto{1}{\ell}} \mid \domelema_j \in A_1, 
\tp{\Lsuffix[\sigma_{\ell{-}1}]}{\str{A}_1}{\domelemtupleafromto{2}{\ell}} = \tp{\Lsuffix[\sigma_{\ell{-}1}]}{\str{B}_1}{\domelemtuplebfromto{2}{\ell}}, \unarytype_{\str{A}_1}(\domelema_j) = \unarytype_j, \mosaicm(\domelema_j) = \mosaicn_j, 1 \leq j \leq \ell
  \big\}.
\]
% $$
Note that $|L| < K$, thus we can enumerate $L$  (possibly with repetitions at the end) as  $\typet_1, \typet_2, \ldots, \typet_K$.
Finally, for any knight $\domelemb_{1} = (((\unarytype, \ldots, c_\ell, \ldots), \mosaicn)$ we interpret $\ell$-ary symbols to fulfil $\tp{\Lsuffix[\sigma_\ell]}{\str{B}_1}{\domelemtuplebfromto{1}{\ell}} = \typet_{c_\ell}$.
This is correct, since $\Lsuffix$ is ``forward'' and $\typet_{c_\ell}$ extends the suffix-type of $\domelemtuplebfromto{2}{\ell}$~in~$\str{A}_1$.\\

\noindent \textbf{Squires.}
Throughout the construction some peasants will be promoted to \emph{squires} (still peasants, but with privileges).
The promotion is done inductively for all $\ell = 1, 2, \ldots, \mas{-}1$.
For all $\ell$-tuples $\domelemtupled \sqin B_1$ of knights and squires\footnote{For $\ell = 1$ we consider only knights, since no peasants were promoted yet.}, unary types $\unarytype$ and $(\sigma,\ell{+}1)$-suffix-types $\typet$ we check if there is an element $\domelema \in A_1$ satisfying the following two conditions:
\begin{itemize}\itemsep0em
  \item $\unarytype_{\str{A}_1}(\domelema) = \unarytype$, $\tp{\Lsuffix[\sigma]}{\str{A}_1}{ \domelemtuplew \domelema } = \typet$, where $\domelemtuplew$ is the $\ell$-tuple of the corresponding witnesses for~$\domelemtupled$
  \item $\domelema \not\sim \domelemg$ for all noble and squire generators $\domelemg$ (defined for smaller $\ell$).
\end{itemize}
In such a case we take some (unpromoted) copy $(\mosaicp, c)$ of a mosaic $\mosaicp = \mosaicm(\domelemd')$ and promote to squires all elements having the form $((\unarytype, \ldots), (\mosaicp, c))$. 
As the generator of $(\mosaicp, c)$ we select any $\domelemg \in A_1 \cup A_2$ witnessing $\domelema \sim \domelemg$, and for every unary type $\unarytype'$ we assign as the witness \emph{for all} elements of the form $((\unarytype, \ldots), (\mosaicp, c))$ any $\domelema' \sim \domelemg$ such that $\unarytype_{\str{A}_1}(\domelema') = \unarytype'$ 
Note that $K$ is \myundef{sufficiently large} so such a free copy of $\mosaicp$ always exists. This concludes the induction.\\

\noindent\textbf{Providing all the remaining connections.}
If some copy $(\mosaicp, c)$ of some plebeian $\mosaicp$ still doesn't have any generator $\domelemg_{(\mosaicp, c)}$ assigned, we simply take as its generator any $\domelemg$ satisfying $\mosaicm(\domelemg) = \mosaicp$. 
Similarly, if there is an element $((\unarytype, \ldots), (\mosaicp, c))$ without having any witness assigned, take as its witness any $\domelema \in A_1$ satisfying $\unarytype_{\str{A}_1}(\domelema) = \unarytype$ and $\domelema \sim \domelemg_{(\mosaicp, c)}$.

Finally, we assign connections between knights and peasants.
We proceed similarly to the previous cases.
Once more, we define $\ell$-ary relations between elements inductively on $\ell \geq 1$ by employing the $c_\ell$ clocks. 
As the case of $\ell = 1$ is already solved, we assume $\ell > 1$.
Take any mosaic $\mosaicm_1 = (\Phi_1, \Phi_2)$, and a unary type $\unarytype_1 \in \Phi_1$.
In case $\mosaicm_1$ is plebeian, we also fix its ``copy number'' $c \leq K$. 
Let $\domelemg_1$ be the generator of $\mosaicm_1$ (in case of noble $\mosaicm_1$) and of $(\mosaicm_1, c)$ otherwise.
Moreover, take $\ell{-}1$ elements $\domelemb_j = ( (\unarytype_j, \ldots), (\mosaicm_j, 
\ldots) \in B_j$, for $2 \leq j \leq \ell$, with the associated generators $\domelemg_j$. 
We stress that some of the selected elements can be knights.
Again, we collect all $(\sigma_\ell,\ell)$-suffix-types that are ``compatible'' with $\domelemtupleb$ by putting $L$ to be the set of suffix-types $\tp{\Lsuffix[\sigma_{\ell}]}{\str{A}_1}{\domelemtupleafromto{1}{\ell}}$ satisfying $\tp{\Linfix[\sigma_{\ell{-}1}]}{\str{A}_1}{\domelemtupleafromto{1}{\ell{-}1}}  = \tp{\Lsuffix[\sigma_{\ell{-}1}]}{\str{B}_1}{\domelemtuplebfromto{1}{\ell{-}1}}$, where for all $1 \leq j \leq \ell$ we have $\domelema_j \sim \domelemg_j$, $\unarytype_{\str{A}_1}(\domelema_j) = \unarytype_j$ and $\domelema_j \in A_1$.
Henceforth we consider only tuples $\domelemtupleb$ containing at least one peasant.
As done before, since $|L| < K$, we can enumerate $L$ (possibly with repetitions at the end) with $\typet_1, \typet_2, \ldots, \typet_K$.
Now, for any peasant $\domelemb_1 = (((\unarytype, \ldots, c_\ell, \ldots), (\mosaicm, c))$ (and analogously for a knight $\domelemb_1 = (((\unarytype, \ldots, c_\ell, \ldots), \mosaicm)$) we interpret $\ell$-ary symbols to fulfil $\tp{\Lsuffix[\sigma_\ell]}{\str{B}_1}{\domelemtuplebfromto{1}{\ell}} = \typet_{c_\ell}$.
Since we extend types in a step-wise manner by taking types that already exist in $\str{A}_1$, by ``forwardness'' of $\Lsuffix$ no conflict occur in the process. We are done by induction.\\

\noindent\textbf{Correctness.}
This concludes the construction of $\str{B}_1$ and $\str{B}_2$.
The satisfaction of \ref{FL:types} is immediate from the construction, and thus we get $\str{B}_1 \models \varphi$ and $\str{B}_2 \models \psi$.\bbeside{Consider extending it...}

Showing \ref{FL:bisim} and that $\str{B}_1 \sim \str{B}_2$ holds is also easy (\bbe{TODO}).
The algorithm deciding IEP amounts to guessing such $\str{B}_1$ and $\str{B}_2$ and verifing their modelhood and bisimilarity, which is clearly feasible in elementary time in $|\str{B}_1|+|\str{B}_2|$.





